Predict the Rover Mobility over Soft Terrain using Articulated Wheeled Bevameter

Robot mobility is critical for mission success, especially in soft or deformable terrains, where the complex wheel-soil interaction mechanics often leads to excessive wheel slip and sinkage, causing the eventual mission failure. To improve the success rate, online mobility prediction using vision, infrared imaging, or model-based stochastic methods have been used in the literature. This paper proposes an on-board mobility prediction approach using an articulated wheeled bevameter that consists of a force-controlled arm and an instrumented bevameter (with force and vision sensors) as its end-effector. The proposed bevameter, which emulates the traditional terramechanics tests such as pressure-sinkage and shear experiments, can measure contact parameters ahead of the rover's body in real-time, and predict the slip and sinkage of supporting wheels over the probed region. Based on the predicted mobility, the rover can select a safer path in order to avoid dangerous regions such as those covered with quicksand. Compared to the literature, our proposed method can avoid the complicated terramechanics modeling and time-consuming stochastic prediction; it can also mitigate the inaccuracy issues arising in non-contact vision-based methods. We also conduct multiple experiments to validate the proposed approach.

==> sections/comments.tex <==
NOTE: 我们做图的目的，是为了更便捷的交流，不是为了好看（当然外观漂亮也是一个重要指标）。
%----------------
【figure-1】
1、first row：
相机换成D435i， T265主要是里程计大鱼眼相机。
右图，加上 which path to choose?
2、middle row
Proposed sinkage and slip ratio prediction ? 感觉没说出重点来；优选下面的
Sinkage and slip ratio prediction using proposed wheeled bevameter
左图：robot arm, wheeled bevameter
中间图： vision-based sinkage detection,  F/T (force/torque) signal
右图：最好换成实际的测量图，而非单轮平台多次试验结果图（花费太多时间了）
3、bottom row
加  safer path (low slip and sinkage)
白色沙子： high slip and sinkage
深色沙子：low slip and sinkage
%---------------

【figure-2】 & 【新figure-3】
【1】单轮平台（现有figure-2），是把robot arm+wheel拆下来之后，安装在单个测试平台上，这里我们想说明的是：方便我们进行大量实验，验证我们所提出的 wheeled bevameter其实是一个很好的测试工具/平台。  多种土壤、多种pressure正压力，多种slip ratio下，测量drawbar pull，driving torque，sinkage， slip ratio等等。   
相当于：我们的机械臂单独拿出来之后，（换个地方/目的，安装在固定架子上），就可以像MIT testbed等来做跟他们类似的实验，实现一物两用。
【2】等它安装在机器人上之后，就相当于一个安装在机器人上的移动实验室（mobile lab on a rover），有点类似于 Mars Science Lab (MSL) 火星车的意思。
【3】把现有的单轮平台图figure-2，当做新的figure-3.  
增加新的figure-2，把figure-1中的rover放大， 整个机器人系统的介绍， mobile platform + arm + wheeled bevameter
%------ 重新考虑一下如何陈述创新------
1、我们的arm+bevameter是一个很好的工具，可放置在机器人上，探测土壤参数（例如，kc, kb, phi, c，需要用到terramechanics的知识）
2、做rover mobility prediction，不需要terramechanics的知识也能达到目的
3、工具放置在静止平台上，代替传统的单轮平台（MIT、日本东北大学）来做实验，一物多用


【figure-3、4，节省空间】

【figure-5】 字太小

【figure-7】把字嵌到图里去，节省空间

【figure-8】  locked wheel sinkage experiment，多次实验总结。 IIT有一篇比较像的，他们是轮子的一部分，只进行下压。

【figure-9】把字嵌到图里去，节省空间
%我们能看到shear相关的数据， driving torque、drawbar pull震荡很大，主要是wheel profile的影响，Canada有一篇论文解释该现象（并不深），用正弦信号来fit

【figure-10、11】，做成左右2个子图，节省空间。

【figure-12、13】，做成左右2个子图，节省空间。

【figure-14】，内容跟figure-1重复，删掉。
